A Comparative Study of Imputation Methods for Multivariate Ordinal Data

Missing data remains a very common problem in large datasets, including survey and census data containing many ordinal responses, such as political polls and opinion surveys. Multiple imputation (MI) is usually the go-to approach for analyzing such incomplete datasets, and there are indeed several implementations of MI, including methods using generalized linear models, tree-based models, and Bayesian non-parametric models. However, there is limited research on the statistical performance of these methods for multivariate ordinal data. In this article, we perform an empirical evaluation of several MI methods, including MI by chained equations (MICE) using multinomial logistic regression models, MICE using proportional odds logistic regression models, MICE using classification and regression trees, MICE using random forest, MI using Dirichlet process (DP) mixtures of products of multinomial distributions, and MI using DP mixtures of multivariate normal distributions. We evaluate the methods using simulation studies based on ordinal variables selected from the 2018 American Community Survey (ACS). Under our simulation settings, the results suggest that MI using proportional odds logistic regression models, classification and regression trees and DP mixtures of multinomial distributions generally outperform the other methods. In certain settings, MI using multinomial logistic regression models is able to achieve comparable performance, depending on the missing data mechanism and amount of missing data.

==> data_description.tex <==
\subsection{VEH: Number of vehicles available}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/VEH.png}}
\caption{pmf of variable VEH.}
\end{figure}


\subsection{MV: When moved into this house or apartment}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/MV.png}}
\caption{pmf of variable MV.}
\end{figure}

\subsection{NP: Number of persons in this household}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/NP.png}}
\caption{pmf of variable NP.}
\end{figure}


\subsection{RMSP: Number of rooms}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/RMSP.png}}
\caption{pmf of variable RMSP.}
\end{figure}

\subsection{ENG: Ability to speak English}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/ENG.png}}
\caption{pmf of variable ENG.}
\end{figure}

\subsection{MARHT: Number of times married}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/MARHT.png}}
\caption{pmf of variable MARHT.}
\end{figure}


\subsection{SCHL: Educational attainment}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/SCHL.png}}
\caption{pmf of variable SCHL.}
\end{figure}

\subsection{RACNUM: Number of major race groups represented}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/RACNUM.png}}
\caption{pmf of variable RACNUM.}
\end{figure}

\subsection{AGEP: Age}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/AGEP.png}}
\caption{pmf of variable AGEP.}
\end{figure}

\subsection{WKL: When last worked}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/WKL.png}}
\caption{pmf of variable WKL.}
\end{figure}

\subsection{PINCP: Total person's income}

\begin{figure}[H]
\centerline{\includegraphics[scale=.2]{figures/data_dict/PINCP.png}}
\caption{pmf of variable PINCP.}
\end{figure}

